Calibration-free IMU-based Relative Orientation Estimation under Dynamic Human Motion

Recent magnetometer-free inertial measurement unit (IMU) methods can reduce drift in joint motion estimation using rigid-body constraints, but they typically require pre-calibrated sensor locations, assumptions of specific joint models (e.g., hinge joints) or limited motion types, or an external reference for global orientation. Furthermore, challenges related to high-frequency impacts (e.g. at foot strikes during gait) and numerical differentiation of noisy measurements have not been explicitly addressed. We propose an extended Kalman filter that estimates relative IMU orientation and sensor location simultaneously, requiring neither offline sensor location calibration nor a global orientation anchor. A systematic simulation study shows that the quality of the relative orientation and the sensor location estimates depends on different motion-intensity sources: the joint center acceleration and the relative angular velocity, respectively. A low-pass filter (LPF) is used to mitigate real-signal outliers before applying the rigid-body constraint. When applied to the OpenSense dataset with real IMU measurements across four subjects with three lower-body joint types during walking and complex tasks including various motion types, the proposed method achieves an overall relative orientation error of 2.61{\deg}, compared with 10.40{\deg} for a baseline using offline-estimated sensor locations and 7.43{\deg} for a baseline using marker-derived sensor locations. These results show that the proposed calibration-free estimation framework handles real IMU data effectively and achieves accurate relative orientation without offline sensor location calibration.

==> chapters/algoritm.tex <==

\section{Method}
\label{sec:algorithm}
\begin{algorithm}
\caption{Calibration-free Joint Orientation and Location Estimation (EKF)}
\textbf{Input:} Filtered accelerometer $\{ \breve{\mathbf{y}}_{a,t}^{S_i} \}_{t=1}^{N}$;
filtered gyroscope copy for $\dot{\boldsymbol{\omega}}$ only $\{ \breve{\mathbf{y}}_{\omega,t}^{S_i} \}_{t=1}^{N}$;
raw gyroscope $\{ \mathbf{y}_{\omega,t}^{S_i} \}_{t=1}^{N}$ for orientation propagation and centripetal term;
initial nominal quaternion estimates $\hat{\mathbf{q}}_{1|1}^{GS_i}$; covariance matrices $P_{1|1}$, $Q$, $R$.
(see Section~\ref{sec:lpf})\\
\textbf{Output:} Orientation estimates $\hat{\mathbf{q}}_{1:N}^{GS_i}$ and
joint-center location vectors $\hat{\tilde{\mathbf{r}}}_i^{S_i}$, for $i=1,2$.
\begin{algorithmic}[1]
\STATE \textbf{for }{$t = 2, \ldots, N $} \textbf{do}
     \STATE \quad \textbf{Time update}
     \STATE\quad $\hat{\mathbf{q}}_{t|t-1}^{GS_i}
           = \hat{\mathbf{q}}_{t-1|t-1}^{GS_i}
             \otimes \exp_q\!\left(\tfrac{T}{2}\,\mathbf{y}_{\omega,t-1}^{S_i}\right)$,
           \quad $i=1,2$
           % \Comment{propagate with \emph{unfiltered} gyroscope (see~\eqref{eq:quat_prop})}
     \STATE \quad$\tilde{\mathbf{r}}_{t|t-1}^{S_i} = \tilde{\mathbf{r}}_{t-1|t-1}^{S_i}$,
           \quad $i=1,2$
           % \Comment{constant-location prediction (see~\eqref{eq:r_rw})}

     \STATE \quad$P_{t|t-1} =  P_{t-1|t-1} + G_{t-1}\, Q\, G_{t-1}^T$

     \STATEx \quad\quad where 
                        $G_{t-1} = \mathrm{blkdiag}\!\left(
                            T\tilde{\mathbf{R}}_{t|t-1}^{GS_1},\;
                            T\tilde{\mathbf{R}}_{t|t-1}^{GS_2},\;
                            \mathcal{I}_3,\;
                            \mathcal{I}_3
                        \right)$ .
    \STATE\quad \textbf{Measurement update}
     \STATE \quad\quad\textbf{Compute filtered joint-center accelerations}
     \STATE\quad\quad $\mathbf{C}_t^{S_i}
           = \left[\mathbf{y}_{\omega,t}^{S_i}\times\right]^2
           + \left[\dot{\breve{\mathbf{y}}}_{\omega,t}^{S_i}\times\right]$,
           \quad $i=1,2$
           % centripetal: raw gyroscope; Euler: filtered gyroscope derivative
           % \Comment{centripetal + angular-acceleration matrix (see~\eqref{eq:C}), filtered}
     \STATE\quad\quad $\mathbf{a}_{jc,t}^{S_i}
           = \breve{\mathbf{y}}_{a,t}^{S_i}
           - \mathbf{C}_t^{S_i}\,\tilde{\mathbf{r}}_{t|t-1}^{S_i}$,
           \quad $i=1,2$
           % \Comment{filtered joint-center acceleration (see~\eqref{eq:ajc})}
     \STATE \quad\quad\textbf{Linearized measurement matrix $H_t$}
    %  \STATE
    % $H_t =
    % \begin{pmatrix}
    %     \left[\tilde{\mathbf{R}}_{t|t-1}^{GS_1}\,\breve{\mathbf{a}}_{jc,t}^{S_1}\times\right] &
    %     -\left[\tilde{\mathbf{R}}_{t|t-1}^{GS_2}\,\breve{\mathbf{a}}_{jc,t}^{S_2}\times\right] &
    %     \tilde{\mathbf{R}}_{t|t-1}^{GS_1}\,\breve{\mathbf{C}}_t^{S_1} &
    %     -\tilde{\mathbf{R}}_{t|t-1}^{GS_2}\,\breve{\mathbf{C}}_t^{S_2}
    % \end{pmatrix}^T$
    % \label{alg:H}
     \STATE\quad\quad \textbf{Innovation}
     \STATE \quad\quad$\mathbf{e}_{\text{link},t}
           = \tilde{\mathbf{R}}_{t|t-1}^{GS_1}\,\breve{\mathbf{a}}_{jc,t}^{S_1}
           - \tilde{\mathbf{R}}_{t|t-1}^{GS_2}\,\breve{\mathbf{a}}_{jc,t}^{S_2}$
           % \Comment{residual of the kinematic constraint~\eqref{eq:constraint}}
     
     \STATE\quad $S_t = H_t\,P_{t|t-1}\,H_t^T + R$
           % \Comment{$S_t \in \mathbb{R}^{3\times 3}$ is the innovation covariance}

     \STATE\quad $K_t = P_{t|t-1}\,H_t^T\,S_t^{-1}$
           % \Comment{$K_t \in \mathbb{R}^{12\times 3}$ is the Kalman gain}

     \STATE\quad $\mathbf{x}_{t|t} = K_t\,\mathbf{e}_{\text{link},t}$
           % \Comment{state correction; prior mean is zero}

     \STATE \quad$P_{t|t} = P_{t|t-1} - K_t\,S_t\,K_t^T$

     \STATE\quad \textbf{Re-linearise}

     \STATE\quad $\hat{\mathbf{q}}_{t|t}^{GS_i}
           = \exp_q\!\left(\tfrac{\boldsymbol{\eta}_{i,t|t}^G}{2}\right)
             \otimes \hat{\mathbf{q}}_{t|t-1}^{GS_i}$,
           \quad $i=1,2$
           % \Comment{$\boldsymbol{\eta}_{i,t|t}^G \triangleq \mathbf{x}_{t|t}[3(i-1){:}3i]$}

      \STATE\quad $\hat{\tilde{\mathbf{r}}}_{t|t}^{S_i}
           = \tilde{\mathbf{r}}_{t|t-1}^{S_i}
           + \delta\tilde{\mathbf{r}}_{i,t|t}^{S_i}$,
           \quad $i=1,2$
           
\textbf{end for}
\end{algorithmic}
\end{algorithm}

The EKF maintains, at each time step $t$, a nominal quaternion $\hat{\mathbf{q}}_{t|t}^{GS_i}$ for each sensor $i \in \{1,2\}$ and a $12 \times 12$ covariance matrix $P_{t|t}$. Let $\tilde{\mathbf{R}}_{t|t-1}^{GS_i} \triangleq \mathbf{R}\!\left(\hat{\mathbf{q}}_{t|t-1}^{GS_i}\right) \in SO(3)$ denote the rotation matrix derived from the predicted nominal quaternion, and let $\mathcal{I}_n$ denote the $n \times n$ identity matrix. The state vector at time $t$ is
\begin{equation}
    \mathbf{x}_t = \begin{bmatrix}
        \boldsymbol{\eta}_{1,t}^G \\[2pt]
        \boldsymbol{\eta}_{2,t}^G \\[2pt]
        \tilde{\mathbf{r}}_1^{S_1} \\[2pt]
        \tilde{\mathbf{r}}_2^{S_2}
    \end{bmatrix} \in \mathbb{R}^{12},
    \label{eq:state}
\end{equation}
where $\boldsymbol{\eta}_{i,t}^G \in \mathbb{R}^3$ is the orientation error perturbation of segment $i$ expressed in the global frame $G$, and $\tilde{\mathbf{r}}_i^{S_i} \in \mathbb{R}^3$ is the joint-center location vector of sensor $i$ in its own sensor frame (defined in~\eqref{eq:r_rw}). The first six components of $\mathbf{x}_t$ correspond to orientation errors and the last six to location vectors. The nominal quaternion $\hat{\mathbf{q}}_{t|t}^{GS_i}$ is maintained separately and updated after each measurement step via re-linearisation.

The process noise covariance is block-diagonal:
\begin{equation}
    Q =
    \begin{pmatrix}
        \boldsymbol{\Sigma}_\omega & \mathbf{0} & \mathbf{0} & \mathbf{0} \\
        \mathbf{0} & \boldsymbol{\Sigma}_\omega & \mathbf{0} & \mathbf{0} \\
        \mathbf{0} & \mathbf{0} & \boldsymbol{\Sigma}_r & \mathbf{0} \\
        \mathbf{0} & \mathbf{0} & \mathbf{0} & \boldsymbol{\Sigma}_r
    \end{pmatrix},
    \label{eq:Q}
\end{equation}
where $\boldsymbol{\Sigma}_\omega = \sigma_\omega^2\,\mathcal{I}_3$ is the gyroscope process noise covariance ($\sigma_\omega = 0.1$~rad/s in our experiments), and $\boldsymbol{\Sigma}_r = \sigma_r^2\,\mathcal{I}_3$ with $\sigma_r^2 = \sigma_\text{link}^2 \times 10^{-9}$ is set very small to enforce a nearly constant joint-center location vector. The measurement noise covariance is $R = \boldsymbol{\Sigma}_{\text{link}} = \sigma_\text{link}^2\,\mathcal{I}_3$, where $\sigma_\text{link}^2 = 1.225$~m$^2$s$^{-4}$ was used in all experiments. Dynamic covariance tuning is outside the scope of this work; per-motion and per-subject optimal values are reported in Figure~\ref{fig:convariance}.


==> chapters/discussion.tex <==
% ============================================================
% Section VI: Discussion
% IEEE Sensors Journal — ~1 column
% Figures used:
%   fig:complex_motion → figures/output/subject04_complex_nowarmup.png
%     Script: _plot_subject04_complex_motion.py
%     Two-panel, post-convergence (t=50–600 s), 30-s rolling window.
%     Top: rolling RMSE for IMU-LPF (green) and IMU-RAW (red dashed).
%     Bottom: gyroscope magnitude |ω| with static (grey) and dynamic
%     (orange) phase shading. Shows ~11 repeated cycles; IMU-LPF
%     oscillates with phases, IMU-RAW shows no correlated recovery.
%   fig:cutoff_sweep → figures/output/cutoff_sweep_overall.png
%     Script: compare_cutoff.py → plot_cutoff_results()
% NOTE: tab:generalization removed — walking/complexTasks numbers
%   are already in tab:main_results (§V-C).
% ------------------------------------------------------------
% PAPER TODOs (open items):
%   1. [Notation consistency] DONE (2026-03-04).
%   2. [Hassan — PSD comparison] Reproduce _plot_imu_psd.py using
%      OpenSim re-simulated IMU data vs. real physical IMU, to show
%      synthetic data lacks broadband STA/impact content.
%      → Replace fig:signal_psd once Hassan provides OpenSim NPZ files.
% ============================================================
% \newpage
% \section{Discussion}
% \label{sec:discussion}

% % -----------------------------------------------------------
% \subsection*{Generalisation and motion-dependent behaviour}
% % -----------------------------------------------------------

% Table~\ref{tab:main_results} shows that IMU-LPF degrades from
% $2.05^\circ$ (walking) to $3.58^\circ$ (complex tasks) —
% a $1.7\times$ increase — while Weygers-mrk degrades from
% $4.77^\circ$ to $9.10^\circ$ ($1.9\times$).
% The LPF advantage therefore \emph{grows} at the harder condition
% ($2.5\times$ vs.\ $2.3\times$): consistent 6~Hz filtering
% suppresses impact artefacts and soft-tissue noise regardless of
% motion type, whereas the unfiltered Weygers framework
% accumulates broadband contamination under multi-planar loads.
% All 18 complex-task trials across three subjects converge
% (outlier-excluded mean $2.98^\circ$, std $0.81^\circ$),
% with no degradation from walking to complex motion for any
% single subject-joint combination.

% The kinematic constraint provides centripetal correction only
% during active motion: at rest,
% $\boldsymbol{\omega}\times(\boldsymbol{\omega}\times
% \tilde{\mathbf{r}}_i^{S_i})\to\mathbf{0}$ and orientation
% integrates from the gyroscope alone, causing slow drift
% consistent with the simulation threshold
% $a_{jc}\gtrsim 1$~m\,s$^{-2}$
% (Section~\ref{sec:sim_observability}).
% Fig.~\ref{fig:complex_motion} illustrates this across the full
% post-convergence trial for Subject~04 (right ankle, complex tasks):
% the rolling RMSE of IMU-LPF oscillates consistently with motion
% phases over $\sim\!11$ repeated cycles —
% rising to $6$--$7^\circ$ during static rest and dropping to
% $3$--$4^\circ$ as soon as dynamic excitation resumes,
% even after a single sit-to-stand transition.
% This confirms that the filter remains within the basin of
% convergence throughout long activity-interrupted sessions.
% IMU-RAW shows no such phase-correlated recovery: its
% stochastically inconsistent innovations mean that renewed
% excitation injects broadband noise rather than tightening
% the constraint, and error fluctuates without systematic
% reduction during dynamic phases.
% NIS for IMU-LPF stays near the $\chi^2_{3,0.05}=7.81$
% threshold throughout, whereas IMU-RAW chronically exceeds it
% during every motion burst — a direct consequence of
% Diagnostics~1--3 in Section~\ref{sec:lpf_justification}.






% -----------------------------------------------------------
% \subsection*{Signal-level analysis and LPF strategy}
% \label{sec:lpf_justification}
% % -----------------------------------------------------------

% The simulation of Section~\ref{sec:simulation} operates under
% the KF's Gaussian assumption and requires no LPF — but real IMU
% signals are fundamentally different.
% Fig.~\ref{fig:psd_sim_real} shows that re-simulated signals
% contain negligible power above 6~Hz, while real walking signals
% exhibit a sustained broadband floor from impact shocks and
% soft-tissue artefacts; this content is absent from the rigid-body
% model and is why the simulation cannot serve as a proxy for
% real-data filter consistency.

% \begin{figure}[tb]
%   \centering
%   \includegraphics[width=\linewidth]{plots/psd_sim_vs_real_2min.png}
%   \caption{Power spectral density of accelerometer signals:
%     OpenSim re-simulation (blue, no ground contact) versus real IMU
%     (Subject~03 walking, red), first 2~min.
%     The re-simulated signals contain negligible power above 6~Hz;
%     real signals show a sustained broadband floor from impact shocks
%     and soft-tissue artefact, absent from the rigid-body model.
%     Dashed: 6~Hz LPF cutoff.}
%   \label{fig:psd_sim_real}
% \end{figure}

% Above 6~Hz, $(2\pi f)^2$ differentiation amplification makes
% the $\dot{\boldsymbol{\omega}}$ noise floor exceed the
% accelerometer PSD by 1--2 orders of magnitude~\cite{Winter1990}
% (Fig.~\ref{fig:signal_psd}), in the same band where soft-tissue
% artefacts concentrate ($9.8 \pm 2.7$~Hz~\cite{Rong2024}).
% Substituting ground-truth states and offsets directly into the
% constraint confirms this is a signal-level problem:
% NIS$\,\approx\!158$ on real data vs.\ NIS$\,\approx\!0.02$ on
% re-simulated signals — 50-fold model violation.
% IMU-LPF restores consistency to NIS$\,\approx\!2.6$
% (Fig.~\ref{fig:constraint_resid}).

% \begin{figure}[tb]
%   \centering
%   \includegraphics[width=\linewidth]{plots/acc_gyr_psd.png}
%   \caption{PSD of accelerometer and $\dot{\boldsymbol{\omega}}$
%     (Subject~03, Knee-R, walking).
%     Above 6~Hz the $\dot{\boldsymbol{\omega}}$ noise floor exceeds
%     the accelerometer PSD by 1--2 orders of magnitude,
%     making the Euler term noise-dominated.}
%   \label{fig:signal_psd}
% \end{figure}

% \begin{figure}[tb]
%   \centering
%   \includegraphics[width=\linewidth]{plots/nis_time.png}
%   \caption{NIS over time (Subject~03, Knee-R, walking).
%     $\mathrm{E[NIS]}=3$ dashed ($\chi^2(3)$).
%     OpenSim re-simulation (blue, $\approx\!0.02$): model holds.
%     Real~+~GT states/offsets (orange, $\approx\!158$): violated.
%     IMU-RAW (red, $\approx\!23$): partially reduced.
%     IMU-LPF (green, $\approx\!2.6$): consistency restored.}
%   \label{fig:constraint_resid}
% \end{figure}

% Table~\ref{tab:lpf_strategies} identifies which terms must share
% bandwidth: centripetal-only filtering gives no improvement
% (7.15$^\circ$ unchanged) because an unfiltered $\dot{\boldsymbol{\omega}}$
% recontaminates the residual.
% Filtering acc and $\dot{\boldsymbol{\omega}}$ together achieves
% $2.90^\circ$; adding centripetal filtering contributes only
% $\Delta = 0.08^\circ$ as $\omega^2 r$ is already band-limited
% by motion dynamics.

% \begin{table}[tb]
%   \caption{%
%     LPF strategy comparison — orientation RMSE (mean $\pm$ std, degrees).
%     Sub02--04, walking + complex tasks, $n = 36$ joint-trials.
%     Best results in bold.
%   }
%   \label{tab:lpf_strategies}
%   \centering
%   \begin{tabular}{lccc}
%     \toprule
%     Strategy & Signals filtered & Overall & Walking \\
%     \midrule
%     No filter        & ---                              & 7.15 $\pm$ 4.31 & 4.52 $\pm$ 2.04 \\
%     Centripetal only & $\boldsymbol{\omega}$ (in $\omega^2 r$) & 7.15 $\pm$ 4.26 & 4.55 $\pm$ 2.07 \\
%     $\dot{\omega}$ only        & $\boldsymbol{\omega}$ (for diff.)   & 4.85 $\pm$ 2.21 & 3.67 $\pm$ 1.68 \\
%     Acc only         & $\mathbf{a}$                     & 5.67 $\pm$ 2.66 & 3.81 $\pm$ 1.78 \\
%     \textbf{Acc + $\dot{\omega}$ (proposed)} & $\mathbf{a}$, $\boldsymbol{\omega}$ (for diff.) & \textbf{2.90 $\pm$ 1.33} & \textbf{2.21 $\pm$ 0.99} \\
%     All                       & $\mathbf{a}$, $\boldsymbol{\omega}$ (all uses) & 2.82 $\pm$ 1.30 & 2.20 $\pm$ 0.97 \\
%     \bottomrule
%   \end{tabular}
% \end{table}



% % -----------------------------------------------------------
% \subsection*{Cutoff-frequency selection and validation}
% % -----------------------------------------------------------

% A 6~Hz cutoff was selected on two physical grounds.
% First, human joint kinematics contain negligible power above
% 6~Hz — the fundamental step frequency is 1--2~Hz with
% harmonics to $\sim\!6$~Hz~\cite{Crenna2021} — so filtering
% below this limit discards valid motion information.
% Second, Fig.~\ref{fig:constraint_resid} shows that real-signal
% model violation (NIS$\,\approx\!158$) is already severe at the
% walking cadence harmonics; 6~Hz sits just below the
% $\sim\!8$~Hz onset of rapid NIS growth, preserving the
% constraint-valid frequency band.

% Fig.~\ref{fig:cutoff_sweep} validates the choice empirically
% by sweeping $f_c$ from 1~Hz to 30~Hz ($n = 42$ trials).
% RMSE forms a flat plateau at 3--6~Hz
% ($2.53^\circ$--$2.68^\circ$, spread $\leq\!0.15^\circ$) and
% degrades steeply above 8~Hz ($3.41^\circ$ at 10~Hz;
% $6.30^\circ$ at 30~Hz, converging to the IMU-RAW level).
% The 6~Hz choice sits at the upper edge of the plateau,
% coinciding with the theoretical motion-bandwidth limit.
% Below 3~Hz, over-filtering attenuates heel-strike harmonics
% that the constraint relies on to estimate joint-centre vectors.
% The histogram shows that 95\% of per-trial optimal cutoffs
% fall at or below 6~Hz, empirically confirming the choice.

% \begin{figure}[tb]
%   \centering
%   \includegraphics[width=\linewidth]{plots/cutoff_sweep_overall.png}
%   \caption{Orientation RMSE vs.\ LPF cutoff frequency for IMU-LPF
%     (mean\,$\pm$\,std; Sub02--04, Sub07).
%     Walking (blue) and complex tasks (red) both plateau between
%     3--6~Hz and degrade steeply above 8~Hz.
%     95\% of per-trial optimal cutoffs fall at or below 6~Hz.}
%   \label{fig:cutoff_sweep}
% \end{figure}


% % -----------------------------------------------------------
% \subsection*{LPF applicability beyond the proposed method}
% % -----------------------------------------------------------

% The LPF requirement extends to the joint-centre estimation task
% itself: Seel's offline identifier~\cite{seel2012joint} applied
% to the same raw signals yields
% $\tilde{\mathbf{r}}_1^{S_1}$ errors of $124 \pm 74$~mm with
% cosine similarity $0.31$ — essentially uncorrelated with the
% true direction, as broadband $\dot{\mathbf{y}}_\omega$
% noise destroys the centripetal cue before any iteration
% can act.
% Applying 6~Hz LPF within the proposed online estimation
% (IMU-LPF) reduces $\tilde{\mathbf{r}}_1^{S_1}$ error to
% $29 \pm 23$~mm (cosine $0.94$) and $\tilde{\mathbf{r}}_2^{S_2}$
% from $48 \pm 38$~mm (cosine $0.70$) to $21 \pm 12$~mm
% (cosine $0.95$), confirming that signal bandwidth alignment
% is a prerequisite for accurate joint-centre estimation
% regardless of whether the method is offline or online.



==> chapters/sec_II.tex <==


\section{Modeling}
\begin{figure}[t]
\centering
% Replace with \includegraphics{filename} later
\includegraphics[width=1\linewidth]{plots/Gemini_Generated_lowerbody_opensense.png}
\caption{NEED UPDATE:(This is a gemini generated plot)Proposed experimental scenario with 5 IMUs configuration and walking+complex motion (use opensim).}
\label{fig:sensor_diagram}
\end{figure}

The model considers two rigid body segments connected by a 3 degrees-of-freedom (DoF) spherical joint without rotational restriction. Let $G$ denote the global (earth-fixed, inertial) frame and $S_i$ ($i\in\{1,2\}$) denote the body-fixed sensor frame rigidly attached to segment $i$. The discrete time index is $t = 1,\ldots,N$, where $N$ is the number of samples and $T$ is the sampling period. As shown in Figure~\ref{fig:sensor_diagram}, the joint-center location vectors $\tilde{\mathbf{r}}_1^{S_1}$ and $\tilde{\mathbf{r}}_2^{S_2}$ — from each sensor frame origin to the joint center, expressed in the respective sensor frame — are \emph{unknown} and estimated online as part of the filter state. The orientation of sensor $i$ is represented by a unit quaternion $\mathbf{q}_t^{GS_i}$, where the superscript $GS_i$ denotes the rotation from frame $S_i$ to frame $G$; the corresponding rotation matrix is $\mathbf{R}_t^{GS_i} \in SO(3)$.

%--------------------------------------------------------------
\subsection{Dynamic Model}
%--------------------------------------------------------------

The notation follows \cite{kok2017using}. The gyroscope measurement for sensor $i$ at time $t$ is
\begin{equation}
    \mathbf{y}_{\omega,t}^{S_i} = \boldsymbol{\omega}_t^{S_i} + \mathbf{e}_{\omega,t}^{S_i},
    \label{eq:gyr_meas}
\end{equation}
where $\boldsymbol{\omega}_t^{S_i} \in \mathbb{R}^3$ is the true angular velocity of segment $i$ expressed in $S_i$, and $\mathbf{e}_{\omega,t}^{S_i} \sim \mathcal{N}(\mathbf{0}, \boldsymbol{\Sigma}_\omega)$ is zero-mean white Gaussian measurement noise with covariance $\boldsymbol{\Sigma}_\omega$.

The orientation quaternion propagates via
\begin{equation}
    \mathbf{q}_{t+1}^{GS_i} = \mathbf{q}_t^{GS_i} \otimes \exp_q\!\left( \frac{T}{2} \bar{\mathbf{y}}_{\omega,t}^{S_i} \right),
    \label{eq:quat_prop}
\end{equation}
where $\otimes$ denotes quaternion multiplication, $\exp_q(\cdot)$ is the quaternion exponential map, and $\bar{\mathbf{v}} \triangleq [0,\, \mathbf{v}^\top]^\top$ denotes the pure-quaternion embedding of a vector $\mathbf{v} \in \mathbb{R}^3$.

The joint-center location vector is modelled as a random walk:
\begin{equation}
    \tilde{\mathbf{r}}_{t}^{S_i} = \tilde{\mathbf{r}}_{t-1}^{S_i} + \mathbf{e}_{r,t}^{S_i},
    \label{eq:r_rw}
\end{equation}
where $\mathbf{e}_{r,t}^{S_i} \sim \mathcal{N}(\mathbf{0}, \boldsymbol{\Sigma}_r)$. A small $\boldsymbol{\Sigma}_r$ encodes the assumption that the physical sensor placement does not change during a trial.

%--------------------------------------------------------------
\subsection{Measurement Model}
%--------------------------------------------------------------

\subsubsection{Kinematic Constraint}


The accelerometer measurement for sensor $i$ at time $t$ is
\begin{equation}
    \mathbf{y}_{a,t}^{S_i} = \mathbf{a}_t^{S_i} + \mathbf{e}_{a,t}^{S_i},
    \label{eq:acc_meas}
\end{equation}
where $\mathbf{a}_t^{S_i} \in \mathbb{R}^3$ is the specific force (true acceleration minus gravitational acceleration) expressed in $S_i$, and $\mathbf{e}_{a,t}^{S_i} \sim \mathcal{N}(\mathbf{0}, \boldsymbol{\Sigma}_a)$ is measurement noise with covariance $\boldsymbol{\Sigma}_a$.


Since both sensor frames are rigidly attached to the same joint, the joint-center acceleration expressed in the global frame must be identical for both segments:
\begin{equation}
    \mathbf{R}_t^{GS_1} \mathbf{a}_{jc,t}^{S_1} = \mathbf{R}_t^{GS_2} \mathbf{a}_{jc,t}^{S_2} + \mathbf{e}_{\text{link},t},
    \label{eq:constraint_phys}    
\end{equation}
where $\mathbf{e}_{\text{link},t} \sim \mathcal{N}(\mathbf{0}, \boldsymbol{\Sigma}_{\text{link}})$ absorbs residual model mismatch, and $\mathbf{a}_{jc,t}^{S_i} \in \mathbb{R}^3$ is the joint-center acceleration expressed in sensor frame $S_i$. Using rigid-body kinematics, $\mathbf{a}_{jc,t}^{S_i}$ is related to the accelerometer reading via
\begin{align}
    \mathbf{a}_{jc,t}^{S_i} &= \mathbf{y}_{a,t}^{S_i} - \mathbf{C}_t^{S_i} \tilde{\mathbf{r}}^{S_i},
    \label{eq:ajc} \\
    \mathbf{C}_t^{S_i} &= \left[\mathbf{y}_{\omega,t}^{S_i} \times\right]^2 + \left[\dot{\breve{\mathbf{y}}}_{\omega,t}^{S_i} \times\right],
    \label{eq:C}
\end{align}
where $[\mathbf{v}\times] \in \mathbb{R}^{3\times 3}$ denotes the skew-symmetric cross-product matrix of vector $\mathbf{v}$, and $\dot{\breve{\mathbf{y}}}_{\omega,t}^{S_i}$ is the angular acceleration obtained by 5-point numerical differentiation of the \emph{filtered} gyroscope signal (see Section~\ref{sec:lpf}); the raw gyroscope $\mathbf{y}_{\omega,t}^{S_i}$ is used for the centripetal term $[\mathbf{y}_{\omega,t}^{S_i}\times]^2$. In previous work \cite{weygers2020drift}, $\tilde{\mathbf{r}}^{S_i}$ is estimated in a separate pre-processing step \cite{seel2012joint}; in the proposed method it is included in the filter state and estimated jointly with orientation.

\subsubsection{Low-Pass Filter Pre-processing}
\label{sec:lpf}
Two physical effects make the raw signals in~\eqref{eq:ajc}
unreliable at high frequencies.
First, numerical differentiation amplifies noise by $(2\pi f)^2$
in power: MEMS gyroscope noise at 10~Hz is amplified
$100\times$ relative to 1~Hz~\cite{Winter1990}, causing
$\dot{\mathbf{y}}_{\omega,t}^{S_i}$ to be noise-dominated
above a few hertz.
Second, real walking signals contain impact shocks and
soft-tissue artefact that violate the rigid-body
assumption~\eqref{eq:constraint_phys} above
$\sim$8~Hz~\cite{Rong2024}.
Both effects corrupt the constraint innovation and degrade
estimation.

Let $f_c = {6}\text{Hz}$ be the cutoff frequency, and let
$\breve{(\cdot)}$ denote the output of a zero-phase 4th-order
Butterworth low-pass filter at $f_c$:
\begin{equation}
    \breve{\mathbf{y}}_{a,t}^{S_i} = \mathrm{LPF}_{f_c}\!\left\{\mathbf{y}_{a,t}^{S_i}\right\},
    \qquad
    \breve{\mathbf{y}}_{\omega,t}^{S_i} = \mathrm{LPF}_{f_c}\!\left\{\mathbf{y}_{\omega,t}^{S_i}\right\}.
    \label{eq:lpf}
\end{equation}
The filtered signals enter~\eqref{eq:ajc}--\eqref{eq:C} selectively:
$\breve{\mathbf{y}}_{a,t}^{S_i}$ replaces the raw accelerometer, and
$\dot{\breve{\mathbf{y}}}_{\omega,t}^{S_i}$ (derivative of the filtered
gyroscope) replaces $\dot{\mathbf{y}}_{\omega,t}^{S_i}$ in the Euler
term.
The raw gyroscope $\mathbf{y}_{\omega,t}^{S_i}$ is retained for the
centripetal term $[\mathbf{y}_{\omega,t}^{S_i}\times]^2$
and orientation propagation~\eqref{eq:quat_prop} to avoid phase
distortion.
Empirical and spectral evidence for the choice of $f_c$ is
provided in Section~\ref{sec:lpf_justification}.



==> chapters/sec_IV_v2.tex <==

\section{Systematic study on simulated dataset}
\label{sec:sim_data}
We first use simulated data to systematically evaluate Alg.~1 under controlled, ground-truth-available conditions, and to characterize how estimation accuracy depends on motion intensity.
\subsection{Simulation Dataset Generation}
% \paragraph{Motion generation}
Synthetic IMU data were generated for the two-segment rigid-body system with $\|{r}_i^{S_i}\|=200$~mm, with the orientation of each $r_i^{S_i}$ drawn randomly. To independently control the two motion excitation sources, relative motion between the segments was generated through random segment angular velocities, while translational motion of the entire system was generated through random linear accelerations of the joint-center. This enabled independent variation of the rotational intensity $I_{\omega}$ and joint-centre acceleration intensity $I_{a_{jc}}$.

Reference segment angular velocities were drawn i.i.d.\ as $\omega_t^{S_i} \sim \mathcal{N}(0, \sigma_{\omega, \text{sim}}^2\mathcal{I}_3)$. The initial ground-truth orientation $q_{1}^{GS_i}$ is parameterized by a random unit axis and an angle $\theta \sim \mathcal{U}(0, 2\pi)$, from which subsequent orientations $q_{2,\dots,t}^{GS_i}$ are integrated via~\eqref{eq:quat_prop} using $\omega_t^{S_i}$.
In each sensor frame , the joint center acceleration $a_{jc}^{S_i}$ is calculated with  $a_{jc}^{S_i} = {{R}_t^{GS_2}}^{-1}(a_{jc}^{G,\text{free}}+{{g}^G})$ where $a_{jc}^{G,\text{free}}$ was simulated as a random cubic spline and is scaled by amplitude $A_{a_{jc}}$ and gravity  is defined as ${{g}^G}=[0,0,-9.82]$~m/s$^2$.
Accordingly, reference sensor acceleration ${a}_t^{S_i}$ was obtained using the rigid body kinematics via~\eqref{eq:ajc}, with ${r_i}^{S_i}$, $\omega_t^{S_i}$, and $a_{jc}^{S_i}$ already generated, and angular acceleration ${\dot{\omega}}_t^{S_i}$ derived by five-point finite differences of ${\omega}_t^{S_i}$.
Sensor signals $\{{y}_{\omega,t}^{S_i}, {y}_{a,t}^{S_i}\}$ were obtained from $\{{\omega}_t^{S_i},a_t^{S_i}\}$ by adding Gaussian noises ($\sigma_a=0.02$~m/s$^2$, $\sigma_\omega=0.2^\circ$/s) and constant per-trial biases (${b}_a\sim\mathcal{U}(\pm\mu_a$~m/s$^2)$ and ${b}_\omega\sim\mathcal{U}(\pm{\mu_\omega}^\circ$/s) with $\mu_a=0.1$ and $\mu_\omega=0.5$), see~\eqref{eq:gyr_meas} and ~\eqref{eq:acc_meas} .

We performed a Monte Carlo simulation comprising 49 scenarios, corresponding to all combinations of seven joint acceleration amplitudes, \(A_{a_{jc}} \in \{0,\,0.05,\,0.1,\,0.5,\,1,\,2,\,10\}\), and seven angular velocity amplitudes, \(\sigma_{\omega,\mathrm{sim}} \in \{0,\,0.01,\,0.1,\,0.5,\,1.0,\,1.35,\,3.0\}\). Each scenario consisted of 10 Monte Carlo realizations of 50\,s of simulated data sampled at 100\,Hz,  resulting in 490 simulation runs in total.


\subsection{Experimental settings and evaluation method}
 The performance of the proposed Alg.~1 is compared against an oracle baseline denoted \emph{Weygers-GT}, which runs the Weygers~\cite{weygers2020drift} orientation filter with ground-truth sensor location vectors $r_i^{S_i}$ supplied directly. This isolates the effect of online $r_i^{S_i}$ estimation: any gap between Alg.~1 and Weygers-GT is attributable to sensor location error, not to the orientation filter itself. Since the simulation approximately matches the assumed Gaussian noise model, no LPF was applied.

The orientation error is evaluated using the root mean squared angular distance (RMSD) between the estimated relative sensor orientation and the ground truth:
$e_q = \sqrt{\frac{1}{N} \sum_{t=1}^{N} d_\angle (\hat{q}_t^{S_1S_2}, q_t^{S_1S_2})^2}$, where $d_\angle(\cdot,\cdot)$ is the angular distance between two quaternions, evaluated over the final 10~s of each trial. The sensor location error calculate the euclidean distance between the ground truth and the final estimate  as $e_{r_i} = \|\hat{r}_{i,final}^{S_i} - r_{i}^{S_i}\|$, where $\hat{r}_{i,final}^{S_i}$ is the state estimate of sensor location at the final time step.

To quantify the motion of the system we use two metrics: the intensity of motion of the whole system at the joint centre $I_{a_{jc}} = \frac{1}{N} \sum_{t=1}^{N} \|a_{jc,t}^{\text{free}}\|$
and intensity of relative rotation of two segments $I_{\omega} = \frac{1}{N} \sum_{t=1}^{N} \|{R}^{S_1 S_2}_t\,\omega_t^{S_2} - \omega_t^{S_1}\|$.

The EKF noise covariances are matched to the simulator noise floor: $\sigma_\omega^2 = (0.2\,\mathrm{deg\,s^{-1}})^2 \approx 1.22\times10^{-5}~\mathrm{rad^2\,s^{-2}}$ in $Q$, and $\sigma_\mathrm{link}^2 = 2 (\sigma_a^2 + \mu_a^2) = 0.0208~\mathrm{m^2\,s^{-4}}$ in $R$. The location process noise is $\sigma_r^2 = \sigma_\mathrm{link}^2 \times 10^{-9}$. The initial state covariance is $P_{1|1} = I_{12}$ and the initial orientation $\hat{q}_{1|1}^{GS_i} = [1,0,0,0]^\top$, and the initial sensor location vector $\hat{r}_{1|1}^{S_i} = [1,1,1]^\top~\mathrm{m}$. The orientation initialization for Weygers-GT is the same as for Alg.~1.


\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{plots/paper_figure/fig2_final.png}
    \caption{
    Alg.~1 vs.\ Weygers-GT orientation error $e_q$ (final 10~s). Each point is one simulation trial; colour encodes $I_{a_{jc}}$. Dashed line: equal performance between two methods.
    }
    \label{fig:sim-aim1}
\end{figure}



\subsection{Result}
\label{sec:sim_parity}

Fig.~\ref{fig:sim-aim1} compares the orientation accuracy of Alg.~1 (which estimates $r_i^{S_i}$ online) against Weygers-GT~\cite{weygers2020drift} (which uses ground-truth $r_i^{S_i}$). At higher joint-centre acceleration intensities (darker points, lower-left of the plot), the two methods achieve nearly identical orientation error, with points clustering along the diagonal. At $I_{a_{jc}} \geq 2$~m/s$^2$, Alg.~1 achieves a median $e_q$ of $1.1^\circ$ compared to $1.5^\circ$ for Weygers-GT, confirming that online estimation of the sensor location vector does not degrade orientation accuracy when the joint-centre acceleration is sufficiently informative. At the lowest tested $I_{a_{jc}}$ levels, orientation errors are large for both methods, consistent with the observability analysis of~\cite{kok2022observability}.


  \begin{figure}[ht]
  \centering
  \includegraphics[width=\linewidth]{plots/paper_figure/fig3_decoupling.png}
      \caption{Alg.~1 estimation error vs.\ motion intensity (420 simulation trials, $I_{a_{jc}} > 0$). Grey dots: individual trials; boxes: interquartile range per intensity level; black line: median trend. Red star (P1): a trial with $e_q = 2.0^\circ$ but $e_{r_1} = 201$~mm; blue diamond (P2): a trial with $e_{r_1} = 0.009$~mm but $e_q = 73^\circ$. Light-coloured dots show all trials in the same corner population (30 for P1, 52 for P2). \textbf{(a)}~$e_q$ vs.\ $I_{a_{jc}}$. \textbf{(b)}~$e_{r_1}$ vs.\ $I_\omega$.}
  \label{fig:sim_2x2}
\end{figure}

Fig.~\ref{fig:sim_2x2} reveals that orientation and sensor location estimation in Alg.~1 are governed by \emph{different} motion intensity parameters. On a log-scale, $e_q$ correlates strongly with $I_{a_{jc}}$ ($R^2 = 0.80$) but not with $I_\omega$ ($R^2 = 0.00$), while $e_{r_1}$ correlates strongly with $I_\omega$ ($R^2 = 0.87$) but not with $I_{a_{jc}}$ ($R^2 = 0.03$). This decoupling is further illustrated by two representative trials highlighted in Fig.~\ref{fig:sim_2x2}: the red-starred trial~(P1) achieves excellent orientation ($e_q = 2.0^\circ$) yet poor sensor location ($e_{r_1} = 201$~mm), because it has high $I_{a_{jc}}$ but near-zero $I_\omega$; conversely, the blue-diamond trial~(P2) achieves excellent sensor location ($e_{r_1} = 0.009$~mm) yet poor orientation ($e_q = 73^\circ$), because it has high $I_\omega$ but low $I_{a_{jc}}$.

Fig.~\ref{fig:sim_2x2}(a) shows that $e_q$ decreases monotonically with $I_{a_{jc}}$, from a median of ${\sim}59^\circ$ at the lowest level ($I_{a_{jc}} = 0.15$~m/s$^2$) to ${\sim}1.3^\circ$ at $I_{a_{jc}} = 29.5$~m/s$^2$. This is consistent with the observability condition derived in~\cite{kok2022observability}: joint-centre acceleration provides the information needed to distinguish relative orientation from sensor-location effects in the accelerometer signal. Fig.~\ref{fig:sim_2x2}(b) shows that $e_{r_1}$ decreases steeply with $I_\omega$; below $I_\omega \approx 0.2$~rad/s the rigid-body constraint cannot resolve all three components of $r_i^{S_i}$ and errors exceed 100~mm.
In summary, the two estimation targets respond to complementary motion characteristics: joint-centre acceleration drives orientation accuracy, while relative angular velocity drives sensor location accuracy.




==> chapters/sec_V_D.tex <==
% ============================================================
% Section V-D: Joint-Centre Offset Estimation Results
% IEEE Sensors Journal — keep SHORT (~0.6 column)
% Numbers from cache: computed via per-joint stats script (n=14 per joint type)
% r2 est/GT values computed 2026-03-03 from kf_final_eval_cache magnitudes
% ============================================================
\subsection{Sensor location estimation}

\label{sec:r1r2}

% In this section, we study the performance of $\hat{r}_i^{S_i}$ for Alg.~1, Alg.~1-no-LPF, and the estimator of sensor location in Weygers~\cite{weygers2020drift} from~\cite{seel2012joint}.

 Having evaluated the relative orientation estimates, we next analyze the  sensor location estimates to interpret the differences in relative orientation  error between the methods. We use the marker-derived vectors  $r_{i,\mathrm{Mrk}}^{S_i}$ as ground truth and compare the locations estimated  by Alg.~1 and Alg.~1-no-LPF with the fixed locations used by  Weygers~\cite{weygers2020drift}, which are obtained using the offline procedure described by Seel et al.~\cite{seel2012joint}.


 % The previous subsection evaluated relative orientation. We now assess the  sensor locations estimated by Alg.~1. We use the marker-derived vectors $r_{i,\mathrm{Mrk}}^{S_i}$ as the ground truth. Figure~\ref{fig:r1r2} compares the errors of  $\hat{r}_i^{S_i}$ from Alg.~1, Alg.~1-no-LPF, and the fixed sensor locations used by Weygers~\cite{weygers2020drift}, which are obtained from the offline procedure described by Seel et al.~\cite{seel2012joint}.  Relative to the marker-derived ground truth, Alg.~1 achieves a mean error of  $60$~mm, compared with $115$~mm for Alg.~1-no-LPF and $134$~mm for the fixed  locations used by Weygers. The difference is most visible at the ankle, where both Alg.~1-no-LPF and the fixed locations used by Weygers exceed  $100$~mm.



\begin{figure}[ht]
\centering
% Replace with \includegraphics{filename} later
% \rule{\columnwidth}{3in} 
    \includegraphics[width=1\linewidth]{plots/paper_figure/fig6_r1r2_pooled.png}
\caption{Sensor location error $e_{r_i}$, averaged over both $i=1,2$, subjects, and left/right sides. The cross-hatched region on the Alg.~1 knee bar indicates the observable perpendicular component following the previous study~\cite{olsson2017experimental}.}

\label{fig:r1r2}
\end{figure} 

Figure~\ref{fig:r1r2} shows that Alg.~1 achieves the lowest mean sensor  location error, $60$~mm, compared with $115$~mm for Alg.~1-no-LPF and  $134$~mm for the fixed locations used by Weygers. Thus, Alg.~1 provides  accurate sensor location estimates online, whereas the fixed locations used by  Weygers are less accurate relative to the marker-derived reference. The  difference is most visible at the ankle, where both Alg.~1-no-LPF and the  fixed locations used by Weygers exceed $100$~mm.

This comparison also helps interpret the orientation results. Weygers and  Weygers-Mrk use the same EKF but different sensor location values, and Weygers has the larger orientation error which can therefore partly be explained by  the less accurate fixed locations used by Weygers.  To isolate the contribution of the LPF, we compare Alg.~1 with   Alg.~1-no-LPF. Removing the LPF increases the mean sensor location error from  $60$~mm to $115$~mm, indicating that the LPF is important for obtaining  accurate online sensor location estimates.



     % These results also help explain the orientation comparison in Table~\ref{tab:main_results}. Weygers and Weygers-Mrk use the same EKF, but Weygers uses the less accurate fixed locations whereas Weygers-Mrk uses the marker-derived locations. The higher orientation error of Weygers can  therefore be partly attributed to its biased sensor location input. Comparing  Alg.~1 with Alg.~1-no-LPF further shows that the LPF is also important for obtaining accurate sensor location estimates.
    
    
     % Figure~\ref{fig:r1r2} allows us to assess whether the sensor location values help explain the orientation results. First, the fixed locations used by  Weygers have a mean error of $134$~mm relative to the marker-derived ground  truth, whereas Weygers-Mrk uses these marker-derived locations directly. Since  both methods use the same EKF, the higher orientation error of Weygers can therefore be partly attributed to its less accurate fixed sensor locations.
 % Next, we analyze the sensor locations estimated by Alg.~1. Alg.~1 achieves a mean error of $60$~mm, compared with $115$~mm for Alg.~1-no-LPF. Because these  methods use the same online estimation framework, this comparison isolates the  effect of the LPF. Removing the LPF substantially increases the error, with the largest difference at the ankle, where both Alg.~1-no-LPF and the fixed locations used by Weygers exceed $100$~mm. Thus, the results indicate that Alg.~1 obtains useful sensor location estimates online, while the LPF is  important for achieving accurate sensor location and orientation estimates.

 We next analyze the joint- and motion-dependent errors of Alg.~1. The ankle  has the lowest mean error ($50$~mm for walking and $47$~mm for complex tasks), followed by the hip ($65$~mm and $55$~mm), whereas the knee has the largest error ($\sim71$~mm for both motion types). The larger knee error is partly  structural: under hinge-like motion, the component of the sensor location vector along the rotation axis is weakly observable~\cite{olsson2017experimental}.  Evaluating only the observable component perpendicular to this axis reduces the knee error to $44$~mm for walking and $41$~mm for complex tasks, as indicated by the cross-hatched region in Fig.~\ref{fig:r1r2}. The corresponding overall mean error decreases from $60$~mm to $51$~mm. The knee error is nearly unchanged between walking and complex tasks  ($70.9$ versus $70.5$~mm), whereas the hip and ankle errors are lower during  complex tasks by $10.2$~mm and $3.6$~mm, respectively. For the two 3-D joints, the ankle has lower error than the hip in both  walking ($50.2$ versus $65.4$~mm) and complex tasks ($46.6$ versus $55.2$~mm), and also has higher mean $I_\omega$ in both motion types. This is consistent  with the simulation result that greater relative angular velocity provides  more information for estimating sensor locations, although differences in joint geometry and marker-based uncertainty may also contribute.

  The joint-wise results further show that relative orientation and sensor location accuracy are not necessarily coupled, consistent with  Section~\ref{sec:sim_result}: the knee has the largest  sensor location error but not the largest orientation error, whereas the hip  has the largest orientation error despite having only a moderate sensor   location error.



% LPF substantially reduces sensor location error. Alg.~1 achieves a  mean $e_{r_i}$ of 60\,mm across all joints, subjects, sides, and both sensors, compared with 115\,mm for Alg.~1-no-LPF and 134\,mm for Seel (Fig.~\ref{fig:r1r2}). The improvement is most visible at  the ankle, where both Alg.~1-no-LPF and Seel exceed 100\,mm,  consistent with stronger heel-strike impacts at this joint. This also connects to the orientation results in Table~\ref{tab:main_results}:  among the two fixed-$r_i^{S_i}$ methods, Weygers performs worse than Weygers-Mrk partly because it relies on less accurate Seel-estimated $r_i^{S_i}$.

% Per joint, Alg.~1 achieves the lowest $e_{r_i}$ at the ankle (50\,mm walking, 47\,mm complex tasks), followed by the hip (65\,mm, 55\,mm),  while the knee is the largest ($\sim$71\,mm for both). The large knee error is partly structural: under hinge-like motion, the component along the rotation axis is weakly observable~\cite{olsson2017experimental}.  Projecting the Alg.~1 knee error onto the observable perpendicular  subspace reduces it to 44\,mm (walking) and 41\,mm (complex tasks),   shown by the cross-hatched region in Fig.~\ref{fig:r1r2}. Replacing the knee's three-dimensional error with its perpendicular component yields an overall observable $e_{r_i}$ reduces from 60\,mm to 51\,mm. The averaged $e_{r_i}$ is broadly similar between walking and complex tasks: knee errors are nearly identical (70.9 vs.\ 70.5\,mm), while hip and ankle errors are lower during complex tasks by 10.2\,mm and 3.6\,mm, respectively. For the 3-D joints, the ankle has lower error than the hip in both walking (50.2 vs.\ 65.4\,mm) and complex tasks (46.6 vs.\ 55.2\,mm), while also having higher mean $I_\omega$ (2.37 vs.\ 2.15\,rad/s for walking and 2.21 vs.\ 1.96\,rad/s for complex tasks). This is directionally consistent with the simulation result that larger $I_\omega$ improves sensor location estimation, but should not be over-interpreted because the trend is not present for every individual subject and the hip and ankle also differ in segment shape, physical $r_{i,\mathrm{Mrk}}^{S_i}$ magnitude and marker-based  uncertainty.

% Within Alg.~1, the knee has the largest $e_{r_i}$ but not the largest $e_q$, while the hip has the largest $e_q$ despite moderate $e_{r_i}$ (Table~\ref{tab:main_results}). These results are consistent with the simulation finding that good orientation accuracy does not necessarily imply good sensor location  estimation. 



\subsection{Additional  complex motion analysis}
\label{sec:case_study}

To characterize Alg.~1 beyond trial-averaged performance, we analyze its  behavior over time under varying excitation levels. We examine a  representative Subject~04 right-hip trial during the complex tasks  (Fig.~\ref{fig:case_study}), which contains intervals of both low and high   motion intensity. This allows us to evaluate how the relative orientation and  sensor location estimates evolve as the excitation decreases and subsequently  increases.


 % To complement the overall results in , we inspect a representative trial from Subject~4, right hip, under complex tasks (Section~\ref{sec:dataset}; Fig.~\ref{fig:case_study}). The trial contains both low- and high- excitation intervals, which makes it useful for showing how Alg.~1 behaves over time.

 % Fig.~\ref{fig:case_study}(a) shows the relative orientation error over the full trial, with the zoomed windows in  Fig.~\ref{fig:case_study}(a-1)--(a-3) highlighting the transition  between low and high $I_{a_{jc}}$. During the stationary interval,  the error remains large because the kinematic constraint is weakly  informative. Once movement resumes, the error drops quickly and then stays bounded. This matches the simulation result in Section~\ref{sec:sim_data}, where orientation accuracy mainly follows $I_{a_{jc}}$.


 Fig.~\ref{fig:case_study}(a) shows the relative orientation error $e_q$ over the full trial, with the zoomed windows in  Fig.~\ref{fig:case_study}(a-1)--(a-3) highlighting the transition  between low and high $I_{a_{jc}}$.  The angular distance stays large during the first 25\,s until sufficient $I_{a_{jc}}$ appears (Fig.~\ref{fig:case_study}(a-1)), consistent with the intensity dependence established in  Section~\ref{sec:sim_data}. During sitting (Fig.~\ref{fig:case_study}(a-2)), $I_{a_{jc}} \approx 0$  renders the kinematic constraint uninformative, letting the gyroscope bias drive slow orientation drift.  Notably, this divergence stops within seconds  when sufficient $I_{a_{jc}}$ resumes (Fig.~\ref{fig:case_study}(a-3)),   suggesting that the method can re-engage the constraint effectively after periods of low intensity.
% The error accumulates when the subject is stationary, but recovers within 

 \begin{figure}[tb]
  \centering
  \includegraphics[width=1\linewidth]{plots/paper_figure/fig6_case_study_subject04_complexTasks_right_hip_no_scatter_abcLabels.png}
  % /home/ruiyuanli/python_driftfree_imuPosition/figures/output/fig6_case_study_subject04_complexTasks_right_hip_no_scatter_abcLabels.png
  \caption{Subject 4, right hip, complex motion. (a) Relative orientation error over the full trial, with the shaded intervals shown in the zoomed views. (b) Estimated sensor location magnitudes over the full trial, with the same zoomed views. Gray curves show the corresponding excitation metrics.}
  \label{fig:case_study}
\end{figure}


  Fig.~\ref{fig:case_study}(b) shows the estimated sensor location  magnitudes $|\hat{r}_i^{S_i}|$ over time. While the relative angular velocity is weak, the estimates remain less settled. As $I_\omega$ increases, both magnitudes converge and then remain stable for the rest of the trial. And once converged, as shown in Fig.~\ref{fig:case_study}(b-2), $\hat{r}_i^{S_i}$ is not changed as defined by the dynamic model and also at the same time little $I_{a_{jc}}$ is applied. Once the motion becomes
  more active, the magnitudes converge and then remain nearly constant
  for the rest of the trial, with only minor fluctuations in the later
  zoomed windows as shown in Fig.~\ref{fig:case_study}(b-3).
  % \caption{Subject 4, right hip, complex motion. (a) Relative orientation error over the full trial, with the shaded intervals shown in the zoomed views. (b) Estimated sensor location magnitudes over the full trial, with the same zoomed views. Gray curves show the corresponding excitation metrics.}

% Fig.~\ref{fig:case_study}(b) shows the convergence behaviour of $|\hat{r}_i^{S_i}|$ over the full trial. Zooming into the first 50 seconds (Fig.~\ref{fig:case_study}(b-1)), $|\hat{r}_i^{S_i}|$ between 10--25 s stays stable but unconverged without angular velocity intensity as shown by the near-0 grey curve. From around 25 s, $|\hat{r}_i^{S_i}|$ responds to the increasing $I_{\omega}$ intensity rapidly and and reaches a steady value within approximately 15\,s. Once $|\hat{r}_i^{S_i}|$ has converged, the magnitudes remain generally stable throughout the rest of the trial regardless of motion type (Fig.~\ref{fig:case_study}(b-2)), with only minor vibration at high angular intensity (Fig.~\ref{fig:case_study}(b-3)).


 % Although $|\hat{r}_i^{S_i}|$ converges and remains stable over the
 %  trial, it does not exactly match the marker-derived reference. For
 %  example, the cross-subject standard deviation is 23\,mm for hip
 %  $r_1^{S_1}$, compared with 7\,mm for the marker reference,
 %  suggesting that the filter uses $r_i^{S_i}$ partly to absorb model
 %  based value, as in Weygers-Mrk-LPF, does not outperform Alg.~1.
% Although the estimated $|\hat{r}_i^{S_i}|$ converges and remains stable, it does not necessarily match the marker-derived ground truth exactly. The cross-subject standard deviation of $|\hat{r}_i^{S_i}|$ (e.g.\ 23\,mm for hip $r_1^{S_1}$) is notably larger than that of the marker reference (7\,mm), suggesting that the filter uses $r_i^{S_i}$ partly as a slack variable to absorb residual model mismatch (soft-tissue artefacts, rigid-body approximation errors) rather than tracking the physical sensor location alone. This also explains why fixing $r_i^{S_i}$ to the marker-based value, as in Weygers-Mrk-LPF, does not outperform Alg.~1 despite using high-precision pre-calibrated vectors: the fixed $r_i^{S_i}$ cannot compensate for model errors, whereas the online estimate can.
